Wavelet Convolutions for Large Receptive Fields

In recent years, there have been attempts to increase the kernel size of Convolutional Neural Nets (CNNs) to mimic the global receptive field of Vision Transformers' (ViTs) self-attention blocks. That approach, however, quickly hit an upper bound and saturated way before achieving a global receptive field. In this work, we demonstrate that by leveraging the Wavelet Transform (WT), it is, in fact, possible to obtain very large receptive fields without suffering from over-parameterization, e.g., for a $k \times k$ receptive field, the number of trainable parameters in the proposed method grows only logarithmically with $k$. The proposed layer, named WTConv, can be used as a drop-in replacement in existing architectures, results in an effective multi-frequency response, and scales gracefully with the size of the receptive field. We demonstrate the effectiveness of the WTConv layer within ConvNeXt and MobileNetV2 architectures for image classification, as well as backbones for downstream tasks, and show it yields additional properties such as robustness to image corruption and an increased response to shapes over textures. Our code is available at https://github.com/BGU-CS-VIL/WTConv.

==> tables/detection_short.tex <==
\begin{table}[ht]
    \centering
    \caption{COCO object detection and segmentation results using Cascade Mask-RCNN \cite{Cai:PAMI:2019:cascademaskrcnn} with different backbones pre-trained on ImageNet-1k using 120/300-epochs schedule, and fine-tuned with 1x/3x schedule. FLOPs are based on an input size of $1280\times800$}
    \begin{tabular}{lccc}
         \toprule
         Configuration         & FLOPs & $\mathrm{AP}^{\mathrm{box}}$ & $\mathrm{AP}^{\mathrm{mask}}$  \\
         \midrule
         \multicolumn{4}{c}{120-epoch pre-train + 1x finetune} \\
         \midrule
         ConvNeXt-T            & 741G & 47.3 & 41.1 \\
         ConvNeXt-T + RepLK    & 776G & 47.8 & 41.4 \\
         WTConvNeXt-T          & 741G & \textbf{47.9} & \textbf{41.5} \\
         \midrule
         \multicolumn{4}{c}{300-epoch pre-train + 3x finetune} \\
         \midrule
         Swin-T         & 745G & 50.4 & 43.7 \\
         ConvNeXt-T     & 741G & 50.4 & 43.7 \\
         WTConvNeXt-T   & 741G & \textbf{51.0} & \textbf{44.4} \\
         \midrule
         Swin-S         & 838G & 51.9 & 45.0 \\
         ConvNeXt-S     & 827G & 51.9 & 45.0 \\
         WTConvNeXt-S   & 827G & \textbf{52.6} & \textbf{45.6} \\
         \bottomrule
    \end{tabular}
    \label{tab:det_short}
\end{table}

==> tables/robustness.tex <==
\begin{table}[ht]
    \centering
    \caption{Classification robustness benchmarks summary.}
    \setlength{\tabcolsep}{8pt}
    \begin{tabular}{lccccc}
         \toprule
         Model           & C $\downarrow$ & $\overline{\mathrm{C}}$ $\downarrow$ & A $\uparrow$ & R $\uparrow$ & SK $\uparrow$ \\
         \midrule
         % Swin-T          & 62.0 & -    & 21.6 & 41.3 & 29.1 \\
         ConvNeXt-T      & 53.2 & 40.0 & 24.2 & 47.2 & 35.1 \\
         WTConvNeXt-T    & \textbf{52.0} & \textbf{38.0} & \textbf{25.3} & \textbf{48.0} & \textbf{35.8} \\
         \midrule
         % Swin-B          & 54.4 & -    & 35.8 & 46.6 & 32.4 \\
         ConvNeXt-B      & 46.8 & 34.4 & 36.7 & 51.3 & 39.4 \\
         WTConvNeXt-B    & \textbf{45.6} & \textbf{32.2} & \textbf{36.9} & \textbf{52.6} & \textbf{39.9} \\
         \bottomrule
    \end{tabular}
    \label{tab:robustness}
\end{table}


==> tables/segmentation.tex <==
\begin{table}[ht]
    \centering
    \caption{ADE20K validation results using UperNet \cite{Xiao:ECCV:2018:upernet} with different backbones pre-trained on ImageNet-1k using 120/300-epochs schedule, and fine-tuned for 80K/160K iterations. FLOPs are based on an input size of $2048\times512$.}
    \begin{tabular}{lccc}
         \toprule
         Configuration                       & Param.     & FLOPs    & mIoU  \\
         \midrule
         \multicolumn{4}{c}{120-epoch pre-train + 80K iterations finetune} \\
         \midrule
         ConvNeXt-T                          & 60M        & 939G     & 44.6     \\
         ConvNeXt-T + RepLK     & 64M        & 975G     & 45.0     \\
         WTConvNeXt-T    & 62M        & 939G     & \textbf{45.4}  \\
         % \midrule
         \midrule
         \multicolumn{4}{c}{300-epoch pre-train + 160K iterations finetune} \\
         \midrule
         Swin-T                              & 60M        & 945G     & 44.5     \\
         ConvNeXt-T                          & 60M        & 939G     & 46.0     \\
         WTConvNeXt-T   & 62M        & 939G     & \textbf{46.6} \\
         \midrule
         Swin-S                              & 81M        & 1038G    & 47.6     \\
         ConvNeXt-S                          & 82M        & 1027G    & 48.7     \\
         WTConvNeXt-S    & 86M        & 1028G    & \textbf{49.0}     \\
         \bottomrule
    \end{tabular}
    \label{tab:semseg}
\end{table}

